Characterization of Matrices Satisfying the Reverse Order Law for the Moore-Penrose Pseudoinverse

We give a constructive characterization of matrices satisfying the reverse-order law for the Moore--Penrose pseudoinverse. In particular, for a given matrix $A$ we construct another matrix $B$, of arbitrary compatible size and chosen rank, in terms of the right singular vectors of $A$, such that the reverse order law for $AB$ is satisfied. Moreover, we show that any matrix satisfying this law comes from a similar construction. As a consequence, several equivalent conditions to $B^+ A^+$ being a pseudoinverse of $AB$ are given, for example $\mathcal{C}(A^*AB)=\mathcal{C}(BB^*A^*)$ or $B\left(AB\right)^+A$ being an orthogonal projection. In addition, we parameterize all possible SVD decompositions of a fixed matrix and give Greville-like equivalent conditions for $B^+A^+$ being a $\{1,2\}$-,$\{1,2,3\}$- and $\{1,2,4\}$-inverse of $AB$, with a geometric insight in terms of the principal angles between $\mathcal{C}(A^*)$ and $\mathcal{C}(B)$.

==> temp.tex <==
m = 400; n = 200; 
rA = 200;  % rank of A, not greater than m and n
N = 100;

test = @(X,A) norm(A*X*A-A) + norm(X*A*X-X) + norm((X*A)'-X*A) + norm((A*X)'-A*X);


dpA = 0; dpinvA = 0; tcond = 0; 
p = 5; q = 5;
for i = 1:N

% UA = orth(rand(m)); VA = orth(rand(n)); 
% SA = zeros(m,n); 
% SA(1:m+1:rA*m+1) = randi(rA,[1 rA]); 
% %SA(1:m+1:rA*m+1) = abs(randn(1,rA)); 
% %SA(1:m+1:rA*m+1) = rand(1,rA); 

% A = UA*SA*VA';
% pA = VA*pinv(SA)*UA';

A = full(sprand(m,n,0.001));


%norm(pinv(A)-pA);
%dpinvA = dpinvA + test(pinv(A),A)/norm(A,'fro');
%dpA = dpA + test(pA,A)/norm(A,'fro');
dpinvA = dpinvA + test(rpinvs(A,p,q),A);
dpA = dpA + test(rpinv_rand_cols(A,p,q),A);


%tcond = tcond + cond(A);
end

dpinvA
dpA
tcond


N = 3000;
tic; for i = 1:N; rpinv(rand(m,n),p,q); end; toc

tic; for i = 1:N; rpinv_rand_cols(rand(m,n),p,q); end; toc



function Arplus = rpinvs(A,p,q)
% rpinv: randomized pseudoinverse of A
[m,n]   = size(A);
[U,S,V] = svd(A);
%P       = randn(m,p);
P = U(:,1:p);
%Q       = randn(n,q);
Q = V(:,1:q);
PTA     = P'*A;
AQ      = A*Q;

Arplus  = pinv(PTA)*(PTA*Q)*pinv(AQ);
